Why You've Got Mail: Evaluating Inbox Privacy Implications of Email Marketing Practices in Online Apps and Services

This study explores the widespread perception that personal data, such as email addresses, may be shared or sold without informed user consent, investigating whether these concerns are reflected in actual practices of popular online services and apps. Over the course of a year, we collected and analyzed the source, volume, frequency, and content of emails received by users after signing up for the 150 most popular online services and apps across various sectors. By examining patterns in email communications, we aim to identify consistent strategies used across industries, including potential signs of third-party data sharing. This analysis provides a critical evaluation of how email marketing tactics may intersect with data-sharing practices, with important implications for consumer privacy and regulatory oversight. Our study findings, conducted post-CCPA and GDPR, indicate that while no unknown third-party spam email was detected, internal and authorized third-party email marketing practices were pervasive, with companies frequently sending promotional and CRM emails despite opt-out preferences. The framework established in this work is designed to be scalable, allowing for continuous monitoring, and can be extended to include a more diverse set of apps and services for broader analysis, ultimately contributing to transparency in email address privacy practices.

==> rebuttal.tex <==
Dataset Availability [R1, R2, R3]:

The database is made available for follow-up papers. We have made the dataset persistent via the Center for Open Science (OSF), and have provided an anonymous and private OSF link below, a DOI will be assigned when we make the OSF repository public after acceptance. \url{https://osf.io/m36t8/?view_only=1c0718a550cd46669e9e58d17784910b}. 

Company Data Protection Guidelines [R1]:

We did not conduct an exhaustive review of each company's data protection guidelines as we felt that this was out of scope. We selected apps and services based on their popularity, and with this popularity comes expectations from end users regarding their privacy. For each service we signed up for, we explicitly checked the boxes, where available, to not have our data shared with third parties. 

No Emails from Certain Companies [R3]:

We cannot causally determine why we did not receive any emails from the remaining 41 services. We can hypothesize that this is because they honored the user's opt-out preferences for sending promotional emails or sharing the user's email with third parties. 

Mitigating Unsolicited Emails [R2, R3]:

We can include some technical and practical solutions to control email-based marketing; we can include discussion about controlling email marketing at the source via regulation as well as at the end-user level. Our results can inform public technology policy by showing evidence that most of the emails are sent through large third-parties, which we do mention in section 5.2, but can elaborate on in the final version. 

We can include further privacy research findings in our discussion in the next revision of the paper. 



-----
Anonymous and private review OSF link during peer review, a DOI will be assigned after acceptance. \url{https://osf.io/m36t8/?view_only=1c0718a550cd46669e9e58d17784910b}

Review 1:

1. It was not verified in detail whether the e-mails received by the services were in line with the published data protection guidelines.

2. Nice study; should be accepted if the database is made available for follow-up papers. Without the database the value of the study is marginal.

Answer Review 1:

Thank you for your review, we authors appreciate your time! 

1. We did not conduct an exhaustive review of each company's data protection guidelines as we felt that this was out of scope. We selected apps and services based on their popularity, and with this popularity comes expectations from end users regarding their privacy. For each service we signed up for, we explicitly checked the boxes, where available, to not have our data shared with third parties. 

2. The database is made available for follow-up papers. We have made the dataset persistent via the Center for Open Science (OSF), and have provided an anonymous and private  OSF link below, a DOI will be assigned when we make the OSF repository public after acceptance. \url{https://osf.io/m36t8/?view_only=1c0718a550cd46669e9e58d17784910b}. 

---

Review 2: 

1. While the above findings are of some interest for privacy research, I believe that the main contribution of the paper is development of the email evaluation framework which should be made available to other researchers. 

2. I think more privacy research findings may improve the paper and bring it to a higher publication-acceptable level.

Answer Review 2:

Thank you for your review, we authors appreciate your time! 

1. The database is made available for other researchers. We have made the dataset persistent via the Center for Open Science (OSF), and have provided an anonymous and private  OSF link during peer review, a DOI will be assigned when we make the OSF repository public after acceptance. \url{https://osf.io/m36t8/?view_only=1c0718a550cd46669e9e58d17784910b}. 

2. We can include further privacy research findings in our discussion in the next version of the paper. 

---

Review 3: 

1. Since the dataset is intuitively free from any PII, can the dataset be released as open source for further studies? 

2. It is unclear why the dataset contains emails from only 109 services/apps. What is the reason for not receiving emails from the remaining 41 services? Please include the details. 

3. Please mention technical remedies and practical solutions to control the email-marketing. Even a simple discussion or tips could be beneficial.

4. The related work (and some of the other sections) can be supplemented with insights from HCI studies that have explored the barriers from the end-user's point of view to stop unwanted emails. Although this aspect is mentioned in the initial sections, a concrete discussion is missing from the paper.

Answer Review 3: 

Thank you for your review, we authors appreciate your time! 

1. The database is made available and released open-source. We have made the dataset persistent via the Center for Open Science (OSF), and have provided an anonymous and private  OSF link below, a DOI will be assigned when we make the OSF repository public after acceptance. \url{https://osf.io/m36t8/?view_only=1c0718a550cd46669e9e58d17784910b}. 

2. We cannot causally determine why we did not receive any emails from the remaining 41 services. We can hypothesize that this is because they honored the user's opt-out preferences for sending promotional emails or sharing the user's email with third parties. 

3 and 4. We can include some technical and practical solutions to control email-based marketing; we can include discussion about controlling email marketing at the source via regulation as well as at the end-user level. Our results can inform public technology policy by showing evidence that most of the emails are sent through large third-parties, which we do mention in section 5.2, but can elaborate on in the final version. 


==> reviewer2.tex <==
This paper explores how popular online services use email marketing to reach their customers. The work is related to privacy in that the authors intended to evaluate which companies sell, share, or leak user email addresses without consent. Their method of data collection does not reveal that any of these companies sold email addresses, but I feel that the assumption this method relies on does not hold in practice. Overall, I do not feel that the paper is a good fit for this track as I feel like the focus is on digital marketing strategies and not privacy.

Pros: P1. I like the idea of studying privacy regulation compliance through email marketing.

Some of the descriptive analyses are useful: P2. 3rd party sender analysis is interesting. However, I would revise the figure to only show relationships between third party senders who work with multiple services.

P3. Clustering services based on their sent emails is an interesting idea. I see how this would be useful for identifying and analyzing the different types of email marketing strategies. However, the execution is poor in this paper (See C3)

P4. Using an LLM to classify the emails is a good idea, but the execution is poor because the method is not validated in any way (see C2).

P4. I feel this paper is a good fit for a marketing/digital marketing journal if the scope is expanded slightly (see C5) and the analyses are done with the revisions discussed in this review (i.e. improve clustering analysis, verify LLM classifications, improve figures). If the authors want this paper to be framed as a privacy paper though, I think a lot more work needs to be done. The entire methodology may be flawed for presenting this as a privacy paper (see C1 and C4).

Cons: C1. I don't believe this paper is really about privacy. a) If there had been evidence of the email being shared with scammers, that may be a privacy finding. However, it is still unclear if GDPR and CCPA are applicable in this research and the authors did not convince me that those legislations are relevant here (e.g. they visit services that are mostly US-based companies, but GDPR applies in the EU). It's definitely possible GDPR and/or CCPA apply, but not enough information is provided in the paper currently. b) Given there is no evidence of the email being shared with scammers, I do not believe the authors can state no privacy violations occur. They make this statement based on the assumption that anyone who obtains the email from the online services (through purchase, sharing agreements, or some form of theft) will send scam emails. However, I do not believe this to be true. In fact, many online services may share the email address of customers with third-party vendors so that their customers can be identified and tracked across the web. This won't result in any scam emails being sent, but certainly will be a violation of customers' privacy. Thus, I find the authors' method useful for studying email marketing campaigns, but less useful for studying privacy.

C2. I think it is possible that an LLM can be used for classifying emails into well-defined categories, but if it hasn’t been done before, the authors should show that the LLM performs well for this task. If it has been done before, provide a citation. I assume it has not, so I suggest the authors have some emails that are manually labeled by an independent researcher/study participants. This labeled validation set can be compared to the labels of the LLM. If the zero-shot LLM gives similar ratings to humans, then you can use on the rest of the emails. If it doesn’t perform well, I would consider few-shot learning.

C3. a) The clustering analysis needs to be improved. The clustering result is not balanced well. There is 1 company in each of cluster 2 and 3, which means it's really not much of a cluster at all. It's just a single observation. Yet, there is a whole description about the characteristics of these two clusters and what types of companies fall into this category. Without stating this is based off of a single observation, I feel it is misleading the reader. Additionally, the remaining three clusters have 2, 9, and 98 companies, respectively. There needs to be more companies in each of the three smallest clusters for this analysis to be useful. b) I can also tell there are problems with this clustering result by looking at Figure 5. The authors use 5 dimensions in their clustering analysis, but Figure 5 shows that the clustering results could be reached by using just two dimensions. I could draw a perimeter around each of the 5 clusters in Figure 5 and almost perfectly separate the 5 groups. This means that the third, fourth, and fifth dimensions are probably adding very little to the result under the current clustering method.

C4. The authors mention CAN-SPAM as an act that should deter unsolicited emails. However, this act specifically states that companies do not need consent to start emailing a person. The act only states that the company must provide an option for the user to stop the emails once they start (e.g. unsubscribe link). Thus, I feel the CAN-SPAM act is not relevant to the current research. The authors could consider testing whether all services provide a way to opt-out of promotional emails and whether they respect this choice.

C5. The authors should expand the scope of their study if they would like the cross-sector analyses (Section 4.5) to be meaningful. Currently, there are only 2 services in the "Financial" category and 1 in "Health". These analyses would be more interesting if more sectors are considered, and there are more services per sector.

Minor comments: Should be "breadth" not "breath" in the last sentence of Section 2. Figure 3 needs better explanation in the text. I didn't find it clear that time series decomposition analysis was being performed and the steps should be better laid out. Only the trend and seasonal figures are referenced in the text.

Questions:
Q1. a)Are there specific sections in GDPR or CCPA that make the authors believe the email marketing practices of companies in the dataset violate these privacy laws?

b) If so, are you positive that CCPA or GDPR apply in this setting? I feel that GDPR likely does not apply to many of these companies as they are not based in the EU.

Q2. What makes the authors feel confident in the assumption that sharing/selling the email would result in spam emails? I believe that emails are more likely to be used for tracking users across the web than for spam.

Q3. Why do some emails fail the SPF/DKIM checks if they are authentically sent by the online service provider that is registered with?

Q4. Why cluster into 5 dimensions when Figure 5 shows that the clusters could be reached (at least almost perfectly) with only 2 dimensions?

Q5. "Additionally, it shows that the weekly seasonal component explains 1.17%

